A Survey of Data Agents: Emerging Paradigm or Overstated Hype?

The rapid advancement of large language models (LLMs) has spurred the emergence of data agents, autonomous systems designed to orchestrate Data + AI ecosystems for tackling complex data-related tasks. However, the term "data agent" currently suffers from terminological ambiguity and inconsistent adoption, conflating simple query responders with sophisticated autonomous architectures. This terminological ambiguity fosters mismatched user expectations, accountability challenges, and barriers to industry growth. Inspired by the SAE J3016 standard for driving automation, this survey introduces the first systematic hierarchical taxonomy for data agents, comprising six levels that delineate and trace progressive shifts in autonomy, from manual operations (L0) to a vision of generative, fully autonomous data agents (L5), thereby clarifying capability boundaries and responsibility allocation. Through this lens, we offer a structured review of existing research arranged by increasing autonomy, encompassing specialized data agents for data management, preparation, and analysis, alongside emerging efforts toward versatile, comprehensive systems with enhanced autonomy. We further analyze critical evolutionary leaps and technical gaps for advancing data agents, especially the ongoing L2-to-L3 transition, where data agents evolve from procedural execution to autonomous orchestration. Finally, we conclude with a forward-looking roadmap, envisioning proactive, generative data agents. A curated companion repository is available at https://github.com/HKUSTDial/awesome-data-agents.

==> metadata.tex <==
\newcommand{\papertitle}{A Survey of Data Agents: Emerging Paradigm or Overstated Hype?
}

\newcommand{\paperrunningauthor}{Y.~Zhu et~al.}
\newcommand{\paperrepository}{https://github.com/HKUSTDial/awesome-data-agents}

\newcommand{\paperauthors}{Yizhang~Zhu\textsuperscript{1},
Liangwei~Wang\textsuperscript{1},
Chenyu~Yang\textsuperscript{1},
Xiaotian~Lin\textsuperscript{1},
Boyan~Li\textsuperscript{1},
Wei~Zhou\textsuperscript{3},
Xinyu~Liu\textsuperscript{1},
Zhangyang~Peng\textsuperscript{1},
Tianqi~Luo\textsuperscript{1},
Yu~Li\textsuperscript{4},
Chengliang~Chai\textsuperscript{5},
Chong~Chen\textsuperscript{7},
Shimin~Di\textsuperscript{6},
Ju~Fan\textsuperscript{4},
Ji~Sun\textsuperscript{2},
Nan~Tang\textsuperscript{1},
Fugee~Tsung\textsuperscript{1},
Jiannan~Wang\textsuperscript{2},
Chenglin~Wu\textsuperscript{8},
Yanwei~Xu\textsuperscript{7},
Shaolei~Zhang\textsuperscript{4},
Yong~Zhang\textsuperscript{2},
Xuanhe~Zhou\textsuperscript{3},
Guoliang~Li\textsuperscript{2,*},
Yuyu~Luo\textsuperscript{1,*}
}

\newcommand{\paperaffiliations}{\textsuperscript{\textbf{*}}\textbf{Corresponding authors:}\\[-0.1em]
\hspace*{0.5em}-- Yuyu~Luo 
(\href{mailto:yuyuluo@hkust-gz.edu.cn}{\texttt{yuyuluo@hkust-gz.edu.cn}})\\
\hspace*{0.5em}-- Guoliang~Li 
(\href{mailto:liguoliang@tsinghua.edu.cn}{\texttt{liguoliang@tsinghua.edu.cn}})
\\[0.2em]
\textsuperscript{\textbf{1}}The Hong Kong University of Science and Technology\\[-0.05em]
\hspace*{0.5em}(Guangzhou), China
\\
\textsuperscript{\textbf{2}}Tsinghua University, Beijing, China
\\
\textsuperscript{\textbf{3}}Shanghai Jiao Tong University, Shanghai, China
\\
\textsuperscript{\textbf{4}}Renmin University of China, Beijing, China
\\
\textsuperscript{\textbf{5}}Beijing Institute of Technology, Beijing, China
\\
\textsuperscript{\textbf{6}}Southeast University, Nanjing, China
\\
\textsuperscript{\textbf{7}}Huawei
\quad
\textsuperscript{\textbf{8}}DeepWisdom
}


==> preamble.tex <==
\usepackage[textwidth=17.4cm,textheight=234mm,top=24mm,columnsep=6mm]{geometry}
\usepackage{amsmath,amsfonts}
\usepackage{newtxtext,newtxmath}
\usepackage{microtype}
\usepackage{graphicx}
\usepackage[table]{xcolor}
\usepackage{array,multirow,rotating,pifont,booktabs,makecell}
\usepackage{enumitem,xspace,stfloats,cite}
\usepackage{caption}
\usepackage{titlesec}
\usepackage{etoolbox}
\usepackage{fancyhdr}
\definecolor{linkpurple}{RGB}{83,52,128}
\definecolor{refteal}{RGB}{0,102,92}
\definecolor{linkblue}{RGB}{0,84,147}
\usepackage[colorlinks=true,linkcolor=refteal,citecolor=linkpurple,urlcolor=linkblue,hyperfootnotes=false]{hyperref}

\makeatletter
\renewcommand{\normalsize}{\@setfontsize\normalsize{10}{12.5}\abovedisplayskip=3mm plus6pt minus4pt\belowdisplayskip=\abovedisplayskip\abovedisplayshortskip=0mm plus6pt\belowdisplayshortskip=2mm plus4pt minus4pt}
\renewcommand{\small}{\@setfontsize\small{8.5}{10}}
\let\footnotesize\small
\renewcommand{\@biblabel}[1]{#1.}
\apptocmd{\@floatboxreset}{\small}{}{}
\patchcmd{\thebibliography}{\list}{\small\list}{}{}
\apptocmd{\thebibliography}{\setlength{\itemsep}{0pt}\setlength{\parsep}{0pt}\setlength{\parskip}{0pt}}{}{}
\makeatother
\normalsize
\setlength{\headheight}{12pt}
\fancypagestyle{paperrunning}{
  \fancyhf{}
  \fancyhead[L]{\small\ifodd\value{page}\papertitle\else\thepage\fi}
  \fancyhead[R]{\small\ifodd\value{page}\thepage\else\paperrunningauthor\fi}
  \renewcommand{\headrulewidth}{0.4pt}
  \renewcommand{\footrulewidth}{0pt}
}
\pagestyle{paperrunning}
\setlength{\parindent}{15pt}
\setlength{\parskip}{0pt plus1pt}
\setlength{\emergencystretch}{2em}
\setlist[itemize]{leftmargin=0.4cm,topsep=1pt,itemsep=0pt}
\setlist[enumerate]{leftmargin=0.6cm,topsep=1pt,itemsep=0pt}

\titleformat{\section}{\normalfont\normalsize\bfseries}{\thesection}{1em}{}
\titleformat{\subsection}{\normalfont\normalsize}{\thesubsection}{1em}{}
\titlespacing*{\section}{0pt}{21dd plus8pt minus4pt}{10.5dd}
\titlespacing*{\subsection}{0pt}{21dd plus8pt minus4pt}{10.5dd}

\renewenvironment{abstract}{\noindent\textbf{Abstract}\enspace\ignorespaces}{\par}
\newcommand{\keywords}[1]{\par\vspace{1ex}\noindent\textbf{Keywords}\enspace\begingroup\def\and{\unskip\enspace\textperiodcentered\enspace}#1\endgroup\par}

\captionsetup{font=normalsize,labelfont=normalfont,labelsep=colon}
\captionsetup[figure]{name=Fig.,skip=3pt}
\captionsetup[table]{skip=5.5pt}

\setcounter{topnumber}{4}
\setcounter{bottomnumber}{2}
\setcounter{totalnumber}{6}
\setcounter{dbltopnumber}{3}
\renewcommand{\topfraction}{0.9}
\renewcommand{\bottomfraction}{0.7}
\renewcommand{\textfraction}{0.1}
\renewcommand{\floatpagefraction}{0.85}
\renewcommand{\dbltopfraction}{0.85}
\renewcommand{\dblfloatpagefraction}{0.85}

\renewcommand{\arraystretch}{1.0}
\definecolor{green}{RGB}{0,128,0}
\definecolor{yellow}{RGB}{255,200,18}
\newcommand{\stab}{\vspace{1.2ex}\noindent}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\stitle}[1]{\stab\noindent{\bf #1}}
\newcommand{\etitle}[1]{\vspace{0.5mm}\noindent $\bullet$ {\underline{\em #1}}}
\newcommand{\ptitle}[1]{\vspace{0mm}{\em #1}}
\newcommand{\ie}{\textit{i.e.,}\xspace}
\newcommand{\eg}{\textit{e.g.,}\xspace}
\newcommand{\greencheck}{{\color{green}\ding{51}}}
\newcommand{\halfcheck}{\color{yellow}\ding{51}\rotatebox[origin=c]{-0.0}{\kern-0.645em\ding{55}}}

\definecolor{githubpurple}{rgb}{0.302,0.165,0.498}
\newcommand{\repositorylink}{{\sffamily\fontsize{10}{12}\selectfont\urlstyle{tt}\href{\paperrepository}{\raisebox{-1.5pt}{\includegraphics[height=10pt]{\paperroot figures/github_icon.png}}\hspace{0.35em}{\bfseries\color{githubpurple}Awesome Data Agents:}\hspace{0.35em}{\color{blue}\underline{\expandafter\nolinkurl\expandafter{\paperrepository}}}}}}

